A Two-dimensional Spatial Optimization Framework for Vehicle Powertrain Systems

This paper presents a modeling framework to optimize the two-dimensional placement of powertrain elements inside the vehicle, explicitly accounting for the rotation, relative placement and alignment. Specifically, we first capture the multi-level nature of the system mathematically, and construct a model that captures different powertrain component orientations. Second, we include the relative element placement as variables in the model and derive alignment constraints for both child components and parent subsystems to automatically connect mechanical ports. Finally, we showcase our framework on a four-wheel driven electric vehicle. Our results demonstrate that our framework is capable of efficiently generating system design solutions in a fully automated manner, only using basic component properties.

==> Report/Titlepage.tex <==
\begin{titlepage}
	\centering
	\vspace*{0.5 cm}
	\includegraphics[width = 120mm]{Figures/Logo.eps}\\[0.5 cm]		% University Logo
	\textsc{\LARGE Eindhoven University of Technology}\\[2.0 cm]% University Name
	\textsc{\Large Master thesis}\\[0.5 cm]							% Course Code
%	\textsc{\large Graduation project}\\[0.5 cm]			% Course Name
	% 	{\bfseries Department of Mechanical Engineering\\}
	\rule{\linewidth}{0.2 mm} \\[0.4 cm]
	{\huge\bfseries Maximum-distance Race Strategies for a Fully Electric Endurance Race Car\\}
	%{\huge\bfseries \hl{Report Title Continuation} \\ }
	\rule{\linewidth}{0.2 mm} \\[1.5 cm]
	
	
	\begin{minipage}{0.4\textwidth}
		% \vspace{0.5cm}
		%\includegraphics[width=0.7\linewidth]{Figures/cover.png}\\[10pt]
		\centering
		% {\Large\bfseries Authors }\\[5pt]
		%\begin{table}[H]
		% \centering
		%   \label{authors}
		
		%  \begin{minipage}{0.4\textwidth}
			\begin{flushright} \normalsize
				
				Master \\
				Department \\
				Research group \\[1cm]
				\emph{Authors}\\
				\textsc{van Kampen} J.H.E.\\[1cm] % Name
			\end{flushright}
		\end{minipage}
		\hspace{1cm}
		\begin{minipage}{0.4\textwidth}
			\begin{flushleft} \normalsize
				
				Automotive Technology \\
				Mechanical Engineering \\
				Control Systems Technology\\[1cm]
				\emph{Student numbers} \\
				0952110\\ %student 
			\end{flushleft}
		\end{minipage}\\[2cm]
		\emph{Supervisor}\\
		dr. ir. M.R.U. Salazar Villalon\\[2cm]
		
		Eindhoven, \today
		
		%\begin{flushright}
		%    \vfill
		%	\hl{Supervised by}\\
		%	\hl{Name, \textsc{TU Eindhoven}}
		%\end{flushright}	
		\newpage
		\includegraphics[width=\linewidth]{Report/Code_of_conduct.pdf}
		\newpage
	\end{titlepage}
